Online and Dynamic Algorithms for Set Cover

In this paper, we study the set cover problem in the fully dynamic model. In this model, the set of active elements, i.e., those that must be covered at any given time, can change due to element arrivals and departures. The goal is to maintain an algorithmic solution that is competitive with respect to the current optimal solution. This model is popular in both the dynamic algorithms and online algorithms communities. The difference is in the restriction placed on the algorithm: in dynamic algorithms, the running time of the algorithm making updates (called update time) is bounded, while in online algorithms, the number of updates made to the solution (called recourse) is limited. In this paper we show the following results: In the update time setting, we obtain O(log n)-competitiveness with O(f log n) amortized update time, and O(f^3)-competitiveness with O(f^2) update time. The O(log n)-competitive algorithm is the first one to achieve a competitive ratio independent of f in this setting. In the recourse setting, we show a competitive ratio of O(min{log n,f}) with constant amortized recourse. Note that this matches the best offline bounds with just constant recourse, something that is impossible in the classical online model. Our results are based on two algorithmic frameworks in the fully-dynamic model that are inspired by the classic greedy and primal-dual algorithms for offline set cover. We show that both frameworks can be used for obtaining both recourse and update time bounds, thereby demonstrating algorithmic techniques common to these strands of research.

==> framework.tex <==
\section{Dynamic Greedy Framework}
\label{sec:framework-full}

In this section, we re-state the greedy framework from~\Cref{sec:framework} to make the following~\Cref{sec:lognlogn-full,sec:logn1-full} self-contained. The reader familiar with the framewoek may skip to the following sections for full proofs of~\Cref{thm:main-update}(i) and~\Cref{thm:main-recourse}(i).

At each time $t$, our algorithm framework maintains a valid solution $\St$ for the active set $\At$ of elements. In addition, it also maintains a mapping of each active element $e \in \At$ to a set $\varphi_t(e) \in \St$ which currently covers it. In a sense, this mapping assigns a unique set to be responsible for covering each element, if multiple sets in $\St$ potentially covers an element. Then, using this mapping, we can associate with each set $S \in \St$, a \emph{current density} which is simply the ratio $\frac{c_S}{|\{e \text{ s.t } \varphi_t(e) = S\}|}$.

Then, the crux of our algorithms is the following {\em stability} property which we maintain at each time $t$: there does not exist a set $S \in \calF$, and a subset of elements $Y \subseteq S \cap \At$ (currently covered in different sets in the solution) such that by adding a new copy of $S$ to $\St$, the current densities of each element in $Y$ \emph{improves (decreases) by a factor of at least $2$}. With this intuition, our high-level algorithmic framework is then the following:

\begin{framed}
\noindent {\bf Element Arrival.} When an element $e$ arrives, buy a new copy of the cheapest set covering the element, and run {\bf Stabilize.}

\medskip \noindent {\bf Element Departure.} When an element $e$ departs, since the current density of the set covering $e$ changes, we run {\bf Stabilize.}

\medskip \noindent {\bf Stabilize.} In this procedure, we check if the current solution is unstable. If it is, we find the set $S$ and subset $Y \subseteq S \cap \At$ of elements so that if we add a new copy of $S$ to the solution $\St$ and make it cover the elements of $X$, each of these elements will improve (decrease) their current density by a factor of at least $2$. We then add this set, and update $\varphi_t(e) = S$ for all $e \in X$. Since this changes the current densities of some sets, we re-run {\bf Stabilize}.
\end{framed}

For the analysis, we use a token scheme. Indeed, each element is initially provided with some number of tokens. Then, whenever we buy new sets in the solution or drop empty sets (which don't cover any elements according to $\varphi(\cdot)$), we will make sure that some tokens are sent out of the system. Then, depending on how the tokens are sent out of the system, we would be able to bound the total amortized recourse or total update time of our algorithm.

Indeed, if we \emph{expend one token per element} which changes its assignment function $\varphi$ whenever we add a new set, this will allow us to bound the total update time, since we can locally bound the time to update the data structures of the solutions in terms of the number of changes to $\varphi$. We describe this algorithm formally in~\Cref{sec:lognlogn}.

On the other hand, for the recourse model, since we only care about the \emph{number} of sets added or deleted,  we would be fine even if several elements which are changing current densities can \emph{collectively expend one token} from the system to pay for the new set we have bought. To incorporate this change, we actually end up refining both our algorithm as well as the analysis. For the algorithm, we will not define current density naively as above, and instead associate a \emph{volume} $\mathsf{vol}\xspace$ for each element which \emph{changes} depending on the current density of the set it is covered by. Then the current density is defined to be the ratio of the cost of the set to the \emph{total volume of elements} it covers. 


==> pseudocode.tex <==
\begin{verbatim}

-----------------------------------------------------------------

Each element remembers:
 - covernode(S) pointer into cov(S) where S covers it
 - the set S covering it (can be figured out from above)
 - level(S), the level i at which it is covered (figured out from above)
 - levelset(e), the chain of f entries in densitylevel_S[level(S)]

Each set S in the solution remembers
 - cov(S)
 - the level at which it is present
Maybe multiple copies of S exist, no problem.

Each set S in \calF remembers:
 - the densitylevel_S[i] for log different levels i.

We also remember
 - unstablelist[i]
 - list of dirty sets

-----------------------------------------------------------------

RemoveElement(e, i):  //Same as you wrote
  e is uncovered, has no level.
  for each S containing e:
    Remove e from densitylevel_S[i], decrement n(S,i)
    if S was unstable and is no longer, remove from unstablelist_i
  end
end  

removeSet(S, X, i):
  remove S from level i
  for e in X:
    removeElement(e,i)
  end
end

insertSet(S, X, i):
  put S at level i
  set cov(S) <- X 
  all elements in X now are covered by S, have level i.
  mark S dirty
end

Stablilize():
  While there exists set S unstable at level i:

    dequeue S from unstablelist[i]

    // Remove the elements from level i
    for e in densitylevel_S(i)
      RemoveElement(e, i)
    end

    // Add in the new set at a lower level
    insertSet(S, densitylevel_S(i), i*) for the right level i^*
    // Remember that new set is dirty

    // Float up the sets
    for all sets S' in S_t (at level i) touched by RemoveElement
      if cov(S') == empty 
        removeSet(S', cov(S'), i)
      else if density-of-set(S') > 2^{i+10}
        removeSet(S', cov(S'), i)
        insertSet(S', cov(S'), i') for the correct level i'
      endif
    endfor

    While there exists (S,i) such that S is dirty at level i:
      handleDirty(S,i)
    endwhile

  endwhile
end

handleDirty(S,i):
  for each element e in cov(S):
    for each S' in sets covering e:
       add e to densitylevel_{S'}[i], update n(S',i), update e's chain 
       if S' is bad, add to unstablelist_i
    end
  end
end

-----------------------------------------------------------------

\end{verbatim}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> qns.tex <==
\section{Things to do}

\begin{itemize}
\item Relate to paper of Lacki, Sankowski, et al.
\item Are streaming algorithms for this problem in the fully dynamic
  settings relavant? E.g., \href{https://arxiv.org/pdf/1610.06199v1.pdf}.
\item Can we get $1-1/e$ for coverage?
\item Can we figure out $2(1+eps)$ for Sayan's proof, even with log update time?
\item Solomon's proof for hypergraphs?
\item Something about this facility location problem?
\end{itemize}


\section{Questions to Resolve}

\begin{itemize}
\item[(a)] Can we make the weighted algorithm non-amortized?
\item[(b)] Can we make it $O(1)$ recourse?
\item[(c)] Can we solve the fractional problem?
\item[(d)] Check if the online facility location extension is easy.. I think so, since we can have exponentially many facilities and still not get hurt in competitive ratio.
\item[(e)] Can we solve the {\em online machine activation problem?} Here, we are given $m$ machines with opening costs $c_i$, and $n$ jobs arrive online. Each job has a running time of $1$ or $\infty$ on these machines, and we're given two bounds $C$ and $T$ on the opening cost, and the makespan on open machines. Can we get $O(\log n) C$, $O(1) T$ bi-criteria algorithms? If all machines are open, then it's like online makespan. If $T = \infty$, then it's like online set cover.
\item[(f)] Can we handle arrivals and deletions?
\item[(g)] Find other applications where we can immediately imply
  improvements?
\item[(h)] Can we also get a result for the dynamic set cover problem,
  where we take care of the running times? Here the main issue is the
  time for Algorithm~{\sf Fix}: every time a new set is bought, we may
  need to update the coverage of many sets, float several sets up,
  etc. Is there a fast data structure to do this, in polylog time?
\end{itemize}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

